Properties of a Bose Gas in the Presence of Disorder (Laurea thesis)

The phenomenon of Bose-Einstein condensation and superfluidity in a Bose gas with disorder is investigated. Diffusion Monte Carlo (DMC) method is used to calculate superfluid and condensate fraction of the system as a function of density and strength of disorder at zero temperature. The algorithm and implementation of the Diffusion Monte Carlo method is explained in details. Bogoliubov theory is developed for the analytical description of the problem. Ground state energy, superfluid fraction and condensate fraction are calculated. It is shown that same results for the superfluid fraction can be obtained in a perturbative manner from Gross-Pitaevskii equation. Ground state energy, obtained from DMC calculations, is compared to predictions of Bogoliubov theory, which are found to be valid in the regime, when the strength of disorder is small. It is shown that "unusual" situation, when the superfluid fraction is smaller than the condensate fraction, can be realized in this system.

==> ref.tex <==
\begin{thebibliography}{99}

\bibitem{Lee Yang}
T.~D.~Lee, K.~Huang, and C.~N.~Yang,
Phys.Rev. {\bf 106}, 1135 (1957)

\bibitem{Crowell}
P.~A.~Crowell, J.~D.~Reppy, S.~Mukherjee, J.~Ma, and
M.~H.~W.~Chan, D~.W.~Schaefer
{\it Critical behavior of superfluid $^4$He films adsorbed in aerogel glass},
Phys. Rev. B, {\bf 51} 12721 (1995)

\bibitem{DMC He}
S.~Giorgini, J.~Boronat, and J.~Casulleras,
{\it Diffusion Monte Carlo study of two-dimensional liquid $^4$He},
Phys. Rev. B {\bf 54} 6099 (1996)

\bibitem{DMC Energy}
S.~Giorgini, J.~Boronat, and J.~Casulleras,
{\it Quantum hard spheres as a model for a homogeneous Bose gas},
Physica B 284-288 (2000)

\bibitem{Aerogel}
Porto, J V et al.,
{\it Suppression of 3He superfluidity by aerogel},
Journal of non-crystalline solids {\bf 225} 205 (1998)

\bibitem{Dirty bosons in 2-D}
N.~Trivedi and M.~Makivic,
{\it In Dirty bosons in 2-D: Phases and phase transitions
Quantum Monte Carlo Methods in Condensed Matter Systems},
M. Suzuki, ed., World Scientific, p. 31 (1993)

\bibitem{Superfluid-insulator transition in disordered boson systems}
W.~Krauth, N.~Trivedi, and D.~M.~Ceperley,
{\it Superfluid-insulator transition in disordered boson systems},
Phys. Rev. Lett., {\bf 67} 2307, (1991)

\bibitem{Quantum Monte Carlo simulations for disordered boson systems}
N.~Trivedi,
{\it Quantum Monte Carlo simulations for disordered boson systems},
In Computer Simulations in Condensed Matter Physics V,
D.~P.~Landau, K.~K.~Mon, and H.~B.~Schuttler, eds., Springer Verlag (1993)

\bibitem{dissertation 1}
Paul Richard Charles Kent,
{\it Techniques and Applications of Quantum Monte Carlo }
(A Ph.D. dissertation),
Robinson College, Cambridge (1999)

\bibitem{dissertation 2}
Andrew James Williamson ,
{\it Quantum Monte Carlo calculations of electronic excitations}
Robinson College, Cambridge (1996)

\end{thebibliography}

